Scaling Compute Is Not All You Need for Adversarial Robustness

The last six years have witnessed significant progress in adversarially robust deep learning. As evidenced by the CIFAR-10 dataset category in RobustBench benchmark, the accuracy under $\ell_\infty$ adversarial perturbations improved from 44\% in \citet{Madry2018Towards} to 71\% in \citet{peng2023robust}. Although impressive, existing state-of-the-art is still far from satisfactory. It is further observed that best-performing models are often very large models adversarially trained by industrial labs with significant computational budgets. In this paper, we aim to understand: ``how much longer can computing power drive adversarial robustness advances?" To answer this question, we derive \emph{scaling laws for adversarial robustness} which can be extrapolated in the future to provide an estimate of how much cost we would need to pay to reach a desired level of robustness. We show that increasing the FLOPs needed for adversarial training does not bring as much advantage as it does for standard training in terms of performance improvements. Moreover, we find that some of the top-performing techniques are difficult to exactly reproduce, suggesting that they are not robust enough for minor changes in the training setup. Our analysis also uncovers potentially worthwhile directions to pursue in future research. Finally, we make our benchmarking framework (built on top of \texttt{timm}~\citep{rw2019timm}) publicly available to facilitate future analysis in efficient robust deep learning.

==> relevant_papers.tex <==
\section{Relevant papers}
\label{sec:rel}

GreenAI:
\begin{itemize}
    \item Energy and Policy Considerations for Deep Learning in NLP \cite{strubell2019energy}
    \item Carbon emissions and large neural network training~\cite{patterson2021carbon, henderson2020towards}
    \item Green AI~\cite{schwartz2020green}: inclusivity (academic labs can't train large models)
    \item Deep learning's diminishing returns~\cite{spectrum}
    \item Compute Trends Across Three Eras of Machine Learning \cite{sevilla2022}
    \item Compute and Energy Consumption Trends in Deep Learning Inference \cite{desislavov2021compute}
    \item Quantization for Sustainable Reinforcement Learning \cite{krishnan2019quarl}
    \item Algorithmic Efficiency and scaling laws \cite{hernandez2020measuring}
\end{itemize}

Performance benchmarks:
\begin{itemize}
    \item MLPerf training benchmark: \cite{mattson2020mlperf}
    \item MLPerf inference benchmark: \cite{reddi2020mlperf}
    \item MLPerf mobile inference benchmark: \cite{reddi2020mlperfmobile}
    \item MLPerf tiny benchmark:  \cite{banbury2021mlperf}
    \item Net Zero Coalition w.r.t. our forecasting
\end{itemize}




%Certified robustness:

%\begin{itemize}
%    \item Certified adversarial robustness via randomized smoothing~\cite{cohen2019certified}
%    \item Integer-arithmetic-only Certified Robustness for Quantized Neural Networks~\cite{lin2021integer}
%    \item SoK: Certified Robustness for Deep Neural Networks~\cite{li2020sok}
%\end{itemize}

%Fast certified robustness:

%\begin{itemize}
%    \item Fast-Lin/Lip~\cite{weng2018towards}
%    \item Crown~\cite{zhang2018efficient}
%    \item alpha-beta-crown~\cite{wang2021beta}
%    \item Look at VNN-Comp-21 for other approaches
%\end{itemize}

%Real use cases of certified robustness/motivation of online certification:

%\begin{itemize}
%    \item In deep RL-based control systems for autonomous vehicles/robots: require fast online certification~\cite{lutjens2020certified}
%    \item Testing and verification of neural-network-based safety-critical control software: A systematic literature review~\cite{zhang2020testing}
%    \item ACAS Xu: Integrated Collision Avoidance and Detect and Avoid Capability for UAS~\cite{owen2019acas}
%\end{itemize}



==> robust_training.tex <==
{

\begin{abstract}
    % \mnote{just an attempt at writing an abstract to see how we can summarize our potential contributions}
    The last five years witnessed significant progress in adversarially robust deep learning. As evidenced by the RobustBench $\ell_\infty$ benchmark, the accuracy under adversarial perturbations got improved from 44\% in \citet{madry2017towards} to 67\% in \citet{rebuffi2021fixing}.
    However, popular benchmarks like RobustBench focus on a single metric and ignore the computational costs needed to train each method which are significant, especially since the best-performing models are often very large models trained by large industrial labs. % often trained using extra data
    % gatekeeping, big companies have an edge?
    Moreover, there have been no systematic studies about the efficiency of these approaches which heavily rely on expensive training procedures and large architectures.
    In this paper, we systematically study the efficiency of adversarially robust models and quantify their environmental and financial costs. We derive \emph{scaling laws for adversarial robustness} which can be extrapolated in future to provide an estimate of how much cost we would need to pay to reach a desired level of performance. This analysis uncover potentially worthwhile directions to pursue in future research. 
    Finally, we make our benchmarking framework (built on top of TIMM) publicly available to facilitate future analysis in efficient robust deep learning.
\end{abstract}



\section{Experimental Setup}
% Finalize datasets, models, and methods that will be interesting to analyze -- 
Goal: achieve diverse performance in terms of factors we will be analyzing. We plan to use pretrained models from RobustBench in addition to these new experiments. 



\subsection{Datasets}
CIFAR-10, ImageNet, maybe CIFAR-100 (rather optional since we'd like to avoid unnecessary experiments, but we can resort to CIFAR-100 if there is no agreement of findings between CIFAR-10 and ImageNet). %\mnote{i'm still a bit doubtful about CIFAR-100 as it will be unlikely to bring much diversity in findings compared to CIFAR-10}



\subsection{Models}
The set of models should be diverse in terms of model size and model complexity. %(total 5 models)
% KB: models to try: ResNet18, Wide-ResNet-28-10, Wide-ResNet-34-10, Wide-ResNet-34-20, Wide-ResNet-50-2, ResNet-50
% in robustbench there's also some slightly different architecture e.g. from https://arxiv.org/abs/2110.03825
We will experiment with following models:

\begin{itemize}
    \item CIFAR-10: ResNet18, WideResNet-28-10, WideResNet-34-10, WideResNet-34-20, EfficientNet-v2, ViTs (with/without ImageNet pretraining), vanilla ViT
    \item ImageNet: EfficientNet-v2, ResNet18, ResNet50, WideResNet-50-2, ViTs (-s, -m)
\end{itemize}
% \mnote{in addition, maybe some compact network such as MobileNet/EfficientNet-v2 would be good to benchmark? since efficiency is the whole point of the paper, it would be strange not to cover efficient architectures.}
% \mnote{@Edoardo: which ViTs precisely would you recommend?}
% This could make sense, although with adversarial pre-training also ViTs (and ViT-like models) could have good performance on CIFAR-10
%Training can tricky 

\subsection{Methods}

\begin{itemize}
\item The set of methods should be diverse in terms of performance (best performing to original low performing methods) and in terms of computational complexity (PGD and advanced methods to fast/free) (total 10 methods)  % \mnote{10 methods is a bit too many, in my opinion})
% Some suggestions: Madry's adversarial training with varying number of steps (2, 5, 10), TRADES, free, FGSM (either with random start, which might not work depending on radius, or GradAlign), adversarial weight perturbation, changing learning rate schedules and number of epochs (e.g. cyclic with few epochs), half precision (not sure whether we want to go into this direction, and it's a bit orthogonal to the others), fine-tuning non robust models (see Jeddi et al. (2020)), weight averaging
% There are also data augmentation (Rebuffi et al. (2021)) and synthetic data, but they do not add computational complexity (apart from generating the synthetic data)
\item For extrapolation in future experiment, we may also want to cover methods from 2017 to 2022 (Figure 1 in \cite{gowal2021improving}). Also do we just want to extrapolate from lowest compute points?
% \item Can we use taxonomy from Table 1 in \cite{bai2021recent} or come up with our taxonomy? \mnote{yes, this is a good list of categories. but maybe we can leave out curriculum-based methods, methods with adaptive $\varepsilon$ and methods with extra unlabeled data.}
\item Do we also want to try extra data approaches? Given complication in collection (and increase in memory) and its diminishing returns.
% Probably collection is not a big deal in the case of labeled data (i.e., pre-training on ImageNet or larger datasets, e.g., Hendrycks et al. (2019)). We can also consider using synthetic data, as mentioned above)
\item This could also be data dependent: computationally expensive methods may not scale to ImageNet.
\end{itemize}


We will experiment with the following methods (\BK{with early stopping using oracle or save model at last epoch with reported hyperprameters or fixed}):
\mnote{update after our discussion: save both the last and the best model (according to the robust accuracy on the test set) and decide latter what to report (but most likely, only the last model)}
% \mnote{To make sure to alleviate robust overfitting, I'd say we should use early stopping for all trained models.} --> update after the discussion: it's controversial how to count training time with early stopping; also, different training schemes may benefit differently from early stopping.
\begin{itemize}
    \item Vanilla adversarial training: multi-step PGD \citep{madry2017towards}
    \item Training objectives: standard adversarial training \citep{madry2017towards}, TRADES \citep{zhang2019theoretically}, possibly 
    % (other candidates: \citep{Qin2019Adversarial} which propose 2 regularizers but I don't think their method really works better; 
    MART \citep{Wang2020Improving} (has been cited 200 times so can be also a reasonable candidate, although I'm not sure it gives a significant improvement upon TRADES)
    \fnote{in principle there shouldn't be much difference between vanilla adversarial training and TRADES except a small improvement in robustness, so maybe varying the number of PGD steps is more interesting} \mnote{I'd say that benchmarking both the vanilla cross-entropy loss and TRADES is valuable. but if we really need to dramatically reduce the number of experiments, we can use only TRADES throughout the paper.}
    \item Flatness-based method: Adversarial Weight Perturbation \citep{wu2020adversarial}
    \item Weight averaging \citep{rebuffi2021data}
    \item Fast Methods: FGSM training \citep{wong2020fast} (\citet{de2022make} recommend to get rid of projection which alleviates catastrophic overfitting), %Adversarial training for free \citep{shafahi2019adversarial}
    % \mnote{i'm not convinced that AT for free works better than FGSM training; + it's not really for free as it actually requires more epochs to train.}
    %\item Ensemble methods: train muliple models (maybe with FGSM to make it reasonable in terms of the training time) with different random seeds and average their predictions.
    %\item Extra data: ImageNet pretraining \mnote{if we do that, we need to reuse the exact same architectures from ImageNet?}
    \item DAWNBench improvements from \citet{wong2020fast}: mixed-precision arithmetics, cyclical learning rates, less training epochs.
\end{itemize}

How to choose learning rate scheduling?
\mnote{important design decision: how do we select hyperparameters for each method? what makes most sense for me: we use the same \textbf{general hyperparameters} for all methods (number of epochs, learning rate, schedule, etc) but use the proposed method-specific hyperparameters (e.g., parameters of the weight averaging). this might lead to a bit suboptimal results for some methods, but i don't think the gap would be significant.}

Also: there are also extra hidden costs due to \textbf{hyperparameter tuning} which are hard to measure precisely. But we can give at least some indication of whether a method is friendly to hyperparameter (like FGSM for which the $\varepsilon$ is fixed) or not (like TRADES for which $\lambda$ has to be tuned -- we will vary $\lambda$). \BK{We will generate pareto-front by varying $\lambda$ instead of tuning/selection}


\section{Metrics to be analyzed}
\subsection{Algorithmic}
Clean accuracy and autoattack robust accuracy (at different $\epsilon$ for $\ell_{\infty}$). %Generalization to unseen attacks?

% \mnote{i'd suggest to focus on a single $\varepsilon$ per dataset. we already have enough of other axes to consider -- good point.}
\begin{itemize}
    \item CIFAR-10 $\epsilon$ levels: $\varepsilon=8/255$
    \item ImageNet $\epsilon$ levels: $\varepsilon=4/255$
\end{itemize}




\subsection{Hardware-related}

% \mnote{inference vs. training time benchmarking -- how do we fit and organize this within a single paper?}
\znote{I'd suggest separating training and inference into two papers - e.g., MLPerf Training and MLPerf Inference. Inference metric can be both HPC and edge focused. Training metric can mainly focus on HPC}

\textbf{Inference}:
\begin{itemize}
    \item Inference time, inference GFLOPs, inference energy 
    % \znote{Do we care about throughput as well?}.
    \item \mnote{benchmark FP8 and FP16 inference?} \znote{add int8 inference as well?} \BK{Will autoattack work with quantized models?}
    \item \mnote{are we interested in benchmarking multiple devices here? and also some inference-time defenses? then inference-time benchmarking can lead to a whole separate paper (although, overlapping with \citet{bhardwaj2022benchmarking}). i'd be actually in favor of this as the inference and training parts are largely independent of each other.} \znote{Benchmarking different devices would be very interesting. And we can classify them based on capacity/scale - data center, edge, mobile, tiny}\BK{This will be a follow up paper. We will briefly discuss some details about this on Friday.}
\end{itemize}

\textbf{Training} (many metrics are sufficient to measure for an epoch only):
\begin{itemize}
    \item Training time, training energy in kilowatt-hour (e.g., see \citep{strubell2019energy}), CO$_2$ emissions of training (e.g., see \citep{henderson2020towards}), USD/epoch (if we use some standard cloud GPUs). \znote{Training has stochastic nature and run-to-run variance. We need to run each scenario multiple times. Probably we can drop the fastest and slowest times, reporting the arithmetic mean of the remaining runs as the result.}
    \item \mnote{benchmark FP8 and FP16 training?} \znote{is FP8 widely used in adversarial training?} \BK{Let us discuss DAWNBench as well.}
    %\item \znote{some methods require re-training, some are not?}
\end{itemize}

\textbf{Static metrics}:
\begin{itemize}
    \item number of parameters \znote{we can make it more hardware-centric? for example, translate number of parameters to memory size}
    \item GFLOPs
\end{itemize}


\section{Analysis questions that we want to answer}
Below are some specific questions we can answer:
\begin{itemize}
    \item {Bhavya to add this next week.}
    \item Based on our analysis we can also develop practical recommendations regarding which techniques promote the idea of green robust AI.
E.g., some methods don't require any extra time and (to be verified) FGSM training is competitive to multi-step approaches, at least for standard $\varepsilon$ accepted in the literature. Moreover, using moderately-sized networks can be good enough in many cases.
\end{itemize}



\section{Analysis methodology that we want to follow}
\begin{itemize}
    \item Objective function for accuracy-robustness trade-off (multiple values of regularizer like in TRADES)
    \item Hyperparameters (fixed epochs or epochs to certain accuracy/robustness?)
    \item Analyzing multi-objective pareto-front and extrapolating: MOO ranking metrics and prediction model for acc/racc
\end{itemize}

}

\section{To do/work plan}
\mnote{Note: if the current number of experiments is too large (esp. on ImageNet), we can benchmark different methods only for a \textbf{single} ResNet, \textbf{single} ViT, and \textbf{single} EfficientNet-v2.}

Use Edoardo's tool for training. (Pls send your github ids to him).

Methods to start with: 1 step, 2 steps and 10 (maybe 7 is better) steps of PGD (\cite{andriushchenko2020understanding}).
Other methods: (i) Does not cause overfitting (\cite{de2022make}), compared to 7 steps PGD.
(ii) Weight averaging (does not require separate training) (\cite{rebuffi2021data}), (iii) Adversarial weight perturbations (\cite{wu2020adversarial}),  (iv) Mixed precision training (\cite{wong2020fast}). \mnote{agreed}

CIFAR-10 models to start with, ask Edoardo about ViTs. 

Just TRADES is fine.

Hardware metrics: Kshitij tried experiment tracker tool (for CO2 emissions) but it didn't give outputs for an example when run on the GPU. Zishen will look more into this.

Evaluate USD cost (\cite{strubell2019energy})

Edoardo has access to TPUs.

\section{To do}
\begin{itemize}
    \item Edoardo to install the adversarial training on lassen
    \item LLNL team will have a shared workspace and install these libraries -- /usr/workspace/robustHW ({\color{blue}{done}})
    \item LLNL team will have a model save/load location (with quota increase): /p/gpfs1/robustHW ({\color{blue}{done}})
    \item LLNL team to download CIFAR-10 and ImageNet and give access: /p/vast1/MLdata ({\color{blue}{done}})
    \item LC/Jupyterhub overview and data access ({\color{blue}{done}})
    \item LC Access {\color{blue}{done}}
    \item LLNL team will integrate hardware metric calculation script with the advtrain library 
    \item Finalize experiments and factors that we want to vary
    \item RobustBench team will write batch training scripts and AutoAttack evaluation scripts
    \item We will then analyze these results and formulate other questions

\end{itemize}

\section{Lassen Commands}
\begin{itemize}
    \item Login: ssh lcname@lassen.llnl.gov and password: pin+RSA
    \item Specific login node: ssh lcname@lassen709
    \item Workspace: cd /usr/workspace/robustHW and install ipython kernel (source bashrc, conda active env, python -m ipykernel install --user --name=env)
    \item Jupyterhub: https://lc.llnl.gov/jupyter/hub/ after using the ipykernel command above
    \item Saved models: cd /p/gpfs1/robustHW
    \item Image Data: cd /p/vast1/MLdata
    \item Make sure you do chmod 770 on all the generated data
    \item Remote editor: atom has support for remote ftp with lassen
    \item Bank: lc.llnl.gov and them to myLC to check bank and other
    \item Debug node: lalloc 1 -q pdebug and bsub -nnodes 1 -q pdebug -W 120 -Is /bin/bash
    \item Check active jobs: lsfjobs -u lcname
    \item Kill a job: bkill jobid
    \item Submit job: bsub job.sh
    \item Share and receive files: give and take
    \item Additional details in the emailed google doc
    \item For our analysis part we may want to look into efficient i/o on LC: \url{https://lc.llnl.gov/confluence/pages/viewpage.action?pageId=660804389}
\end{itemize}


\section{To do: July 15th week}
\begin{itemize}
    \item Edoardo: Integrate weights and biases, Maksym's autoattack implementation, test TRADES
    \item Kshitij and Bhavya: Finalize other hardware metrics (training flops)
    \item Zishen: Finalize scripts to compute train cost after training
    \item All: Finalize experiments to run next week
    \item Venue and timeline
\end{itemize}

\section{To do: August 8th week}
\begin{itemize}
    \item Bhavya: Explore weights and biases and Automatic Chaining (done)
    \item Edoardo: Maksym's autoattack implementation (done), test TRADES
    \item Integrated Hardware Metrics: CO2 emission, latency/time, training flops, training cost, energy cost (done)
    \item Vikash: Training flops in the backward pass of adversarial training may be tricky (done)
    \item Edoardo: Use ViTs with differentiable upsampling on CIFAR-10
    \item Add additional training methods
    \item All: Finalize experiments to run next week
\end{itemize}

\section{To do: August 22nd week}
\begin{itemize}
    \item Bhavya: look into dataparallel issue
    \item Edoardo: implement ViTs with differentiable upsampling (and different resolutions), other training methods, TRADES hyperparameter
    \item Integrate pretraining cost in our code (posthoc)
    \item Maksym and Vikash: Finalize experiments to run next week
\end{itemize}

\section{To do: August 29nd week}
\begin{itemize}
    \item Use early stopping
    \item Edoardo: implement ViTs with differentiable upsampling (and different resolutions), other training methods, TRADES hyperparameter
    \item Integrate pretraining cost in our code (posthoc)
    \item All: Finalize experiments and analysis method
\end{itemize}

\section{To DO: October 15th week}


\begin{itemize}
    \item Chaining large batch jobs: failed in LSF. Contact LC. 
    \item Fix NaN CO2 issue: Zishen will look into the file writing issue. Done.
    \item Units (and transformations) for hardware metrics. 
    \item Finalize factors for neural scaling laws for adversarial robustness. 
    \item Which loss should we use for scaling analysis?
    \item Look at the range of both robust and  clean accuracy to make sure they are sufficiently diverse.
    \item Which interventions to try to improve robustness: deeper, wider, more or less epoch with LR schedule change, more or less data, pretraining, etc.
    \item Add RobustBench training methods: complete analysis vs. 1 epoch. Which methods to add? Weight averaging and adversarial weight perturbation with TRADES first. 
    \item Finalize different fits to compare: polynomial, extrapolation, exponential, etc. Note that we have two dependent target variables. 
\end{itemize}

\section{To DO: October 22nd week}

\begin{itemize}
    \item Add RobustBench training methods: complete analysis vs. 1 epoch. Which methods to add? Weight averaging and adversarial weight perturbation with TRADES first. 
    \item Email LC support for weights and biases. Resolved.
    \item Generative model. Discuss with Vikash. 
    \item Bigger architecture: WideResNet-70-16
    \item How to evaluate CO2 emission for extra data? 1 epoch vs from scratch or don't include given it is a one-time cost. 
    \item Which interventions to try to improve robustness: deeper, wider, more or less epoch with LR schedule change, more or less data, pretraining, etc.
    \item Finalize different fits to compare: polynomial, extrapolation, exponential, etc. Note that we have two dependent target variables. 
\end{itemize}

\section{Neural Scaling Laws for Adversarial Robustness: references and thoughts}
We benchmark the extent of adversarial ML's compute dependency, showing that progress across a wide variety of applications is strongly reliant on increases in computing power. Extrapolating forward this reliance reveals that progress along current lines is rapidly becoming economically, technically, and environmentally unsustainable.

\subsection{Questions to be answered}
In the adversarial robustness context, we aim to answer the question below.
\begin{itemize}
    \item Analysis of the compute growth (or doubling rate) with year for RobustBench models? Similar to Figure 1 in \cite{rebuffi2021fixing} but with compute metrics.
    \item \textbf{MAIN QUESTION:} What are neural scaling laws for adversarial robustness? This could be derived for different scenarios as in \cite{kaplan2020scaling} Sec 6 etc.
    \item What is driving adversarial robustness advances---compute or algorithmic innovations? Similar to \cite{thompson2020computational} by using a conditioning variable. 
    \item Forecasting the future: what would be the economic and environmental costs for achieving 70 or 75\% robust accuracy (or a certain benchmark level for a given application such as AV)? 
    \item Compare these results with common statistics from \cite{strubell2019energy, lohn2022ai}: Air travel, Human life, US GDP, NIF, etc.
    \item Where will future advances come from?: Predicting the most effective interventions by fitting a model that takes this information as input. 
    \item Compare findings with \cite{huang2021exploring}: more parameters (higher model capacity) do not necessarily help adversarial robustness.
    \item What are ethics and policy considerations? These relationships will allow us to determine the optimal solution of a fixed compute budget, etc.
\end{itemize}

\subsection{Notes and Relevant References}
\noindent\textbf{Data Fitting Method:} Multivariate regression vs constrained prediction? Pointwise estimates vs uncertainty-aware (conformal) prediction? Do we want to predict performance as a function of interventions?

\noindent\textbf{Power Law Scaling:}\footnote{\url{https://github.com/MIT-FutureTech/TheComputationalLimitsOfDeepLearning}} \cite{thompson2020computational} used high order polynomial (vs. exponential) as the fitting function, i.e., $\log_{10}(1/error) = \alpha + \beta \times \log(computation)$. They also report  OLS Regression and Quantile Regression results for different scenarios such as only analyzing best models. Using quantile regression, they estimate the scaling at the threshold of the 10\% most efficient models while accounting for algorithmic improvement using  a time trend as a proxy. They also extrapolate the estimates to understand the projected computational power needed to train models to hit various benchmark performance levels. To make these targets tangible, they present them not only in terms of the computational power required but also in terms of the economic and environmental cost of training such models on current hardware.

One can also use extrapolation loss based estimators to fit scaling law \cite{alabdulmohsin2022revisiting} using the method in A.1: To predict the benefit of scale empirically, we argue for a more rigorous methodology based on the extrapolation loss, instead of reporting the best fitting (interpolating) parameters.

\subsection{Driving Factors for Current Adversarial Robustness Research}
We can analyze with RobustBench data for motivating our work: 
1) how is the model size (or costs) growing over time to achieve better performance and maybe we see different eras of adversarial deep learning? The regressions and doubling rates are derived from log-linear fits to the training compute and evaluated in terms of goodness of fit, e.g., R2 score. The amount of compute used to adversarially train deep learning models has increased 300,000x in 5 years and the doubling rate in training compute and trainable parameter counts are increasing for different eras. 

With our data, we carry out a more systematic analysis to analyze the effects of various interventions to answer:

1) Projection\footnote{\url{https://github.com/georgetown-cset/AI_and_compute_2022}} \cite{lohn2022ai, thompson2020computational}: note that compute per dollar is dependent on hardware advances, thus, we should provide uncertainty similar to Figure 2 in  \cite{lohn2022ai}. 

2) We can ask extrapolation questions such as: how much compute is required to reach 70\% robust accuracy (flops vs accuracy)? and what would robust accuracy and training costs be in 2025 (year vs accuracy)?

3) Compare these results with common statistics from \cite{strubell2019energy, lohn2022ai}: Air travel, Human life, US GDP, NIF, etc.

4) Where will future advances come from?: Predicting most effective interventions by fitting a model that takes this information as input. 



Diminishing returns of existing robustness interventions: Progress is becoming increasingly infeasible as compute requirements are growing faster than progress in computing hardware.


\subsection{Neural Scaling Laws for Robustness}
Inspired from \cite{kaplan2020scaling}: We study empirical scaling laws for adversarial robustness on the cross-entropy loss and 0-1 error on test data. The loss is expected to scale as a power law with model size, dataset size, and the amount of computing used for training. Other architectural details such as network width or depth may have minimal effects within a wide range. Simple equations will govern the dependence of overfitting on model/dataset size and the dependence of training speed on model size. These relationships will allow us to determine the optimal allocation of a fixed compute budget. When training within a fixed compute budget C, but with no other constraints, our equation will lead to the prediction that the optimal model size N, optimal batch size B, optimal number of steps S, and dataset size D. Power-law exponents for the scaling of the loss as $L(X) \propto 1/X^{\alpha_X}$ where X can be any of the factors, e.g., parameters, compute, etc. 

\newpage



\section{Measuring the impact of Robust training on carbon emissions}
\label{sec:robust_training}

What is the extra cost of robust training over standard training? Metrics to evaluate on Lassen: training time per epoch, GPU power consumed per epoch. Evaluate carbon emissions using these metrics and compare with standard training. 

We should choose our representative adversarial training methods (on \textbf{CIFAR-10/100, ImageNet}) to 1) cover methods from 2014 to 2022 (Table 1 in \cite{gowal2021improving} or \cite{croce2020robustbench}), 2) cover methods from different adversarial training categories from Table 1 in \cite{bai2021recent}, and 3) are state-of-the-art \cite{croce2020robustbench}. 

We can analyze these different categories in terms of different metrics~\cite{hendrycks2021pixmix}. We will need to be careful about which code/attack we use to calculate robust accuracy. AutoAttack (from RobustBench) is the gold-standard, however, may not have performance for all the models and attack levels that we want to characterize. An ideal study would be where we analyze these adversarial training algorithms by varying different knobs: model type/size, attack strength in AutoAttack \mnote{I think we should have a single standardized attack throughout the paper, otherwise the robustness numbers will be incomparable}, etc. Unfortunately, this will require careful hyperparameter tuning and full training for evaluation -- we can choose hyperparameters from existing papers (make a list of different models from these papers that use AutoAttack). We should take these considerations into account while choosing our methods.

\begin{itemize}
    \item Vanilla/Benchmark: (old, mid, new) and SOTA
    \item Regularization: papers with code:~\cite{goodfellow2014explaining}, \cite{kurakin2016adversarial}, \cite{zhang2019theoretically}, \cite{wang2019improving} \mnote{not sure about \cite{goodfellow2014explaining, kurakin2016adversarial} as their robustness evaluation isn't fully conclusive. maybe let's start from \cite{madry2017towards}?}
    \item Ensemble: papers with code:~\cite{tramer2017ensemble}, \cite{pang2019improving}, \cite{yang2020dverge} \mnote{I think benchmarking ensembles can be done rather briefly (maybe only the standard ensembling scheme, i.e. averaging the predictions). I don't think there is evidence that ensembles are helping a lot but they obviously linearly increase both training and inference time which makes them less competetive in the accuracy-runtime tradeoff.}
    \item Efficient: papers with code:~\cite{shafahi2019adversarial}, \cite{wong2020fast}, \cite{kim2020understanding}, \cite{andriushchenko2020understanding}, \cite{vivek2020regularizers}
\end{itemize}

{\bf Some of the old and new robust training algorithms to compare that are on robustbench (codes available), from 2019-22:} Can we categorize these in terms of the above categories?



\begin{itemize}
    \item Robust training time vs. standard training time: CIFAR10 and ImageNet (2 plots)
    \item Robust training time breakdown (conv/BN layers) vs. standard training time breakdown: CIFAR10 and ImageNet (2 plots) \mnote{what is meant here by "conv/BN layers"? an ablation study where we remove BN from the network? i guess this could be a bit problematic as it would make some (most?) architectures untrainable}
    \item Robust training power vs. standard training power: CIFAR10 and ImageNet (2 plots)
    \item Carbon emission comparisons: CIFAR10 and ImageNet (2 plots)
\end{itemize}
\vnote{I am afraid that the trend in all these plots is likely that robust training incurs linearly higher cost compared to standard training, something that is well known. Then the novelty here is that we measure/uncover this trend for metrics like power or carbon emission, but will it be enough? In a way both these metrics are tied to training cost, which almost linearly depends on number of attack steps.}

{\bf Which conference or workshop?}

Nature Comms, IEEE spectrum, JMLR/Communications of the ACM, MLSys (deadline in October).


{\bf Types of experiments performed in earlier Green AI works:}

\begin{itemize}
    \item In~\cite{patterson2021carbon}, CO2 emissions for different types of NLP models (old and new) and hardware (GPU vs. TPU). Also compared to CO2 emissions of airlines; detailed analysis of FLOPS, power, energy consumed vs. the number of parameters for different models; asks a key question at the end: Are the benefits of NLP models worth the energy cost? 
    \item In~\cite{schwartz2020green}, a graph on how many papers target only accuracy, how many also efficiency, and how many both?; a graph on diminishing returns of training on more data; also presents FLOPs analysis vs. accuracy for different models (old and new).
    \item In~\cite{spectrum}, a projection graph on how by 2025, ImageNet accuracy will improve just by 5\% as the models get more complex (in terms of FLOPS) but this comes with a massive increase in CO2 emissions (also compares to NYC emissions). Such a study for roobustness will be very interesting as SOTA is pretty bad.
\end{itemize}
